TaylorGAN: Neighbor-Augmented Policy Update for Sample-Efficient Natural Language Generation

Score function-based natural language generation (NLG) approaches such as REINFORCE, in general, suffer from low sample efficiency and training instability problems. This is mainly due to the non-differentiable nature of the discrete space sampling and thus these methods have to treat the discriminator as a black box and ignore the gradient information. To improve the sample efficiency and reduce the variance of REINFORCE, we propose a novel approach, TaylorGAN, which augments the gradient estimation by off-policy update and the first-order Taylor expansion. This approach enables us to train NLG models from scratch with smaller batch size -- without maximum likelihood pre-training, and outperforms existing GAN-based methods on multiple metrics of quality and diversity. The source code and data are available at https://github.com/MiuLab/TaylorGAN

==> figures/rnn_workflow.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/rnn_workflow-2.png}
    \captionof{figure}{Generator}
    \label{fig:rnn-workflow}
\end{figure}


==> tables/coco_comparison.tex <==
\caption{
    FED \& LM scores on COCO. Lower is better. Batch size $N=64$ if not specified. $\dagger$ follows the settings of \protect\cite{ScratchGAN} and $\ddagger$ are pre-trained by MLE.
}
\label{tab:fed_lm_score}
\vspace{2mm}
\centering
\begin{tabular}{lrrc}
    \toprule
    \multirow{2}{*}{\bf Model}  & \multicolumn{2}{c}{\bf FED} & \bf LM \\
    \cmidrule{2-3}
    % \cline{2-3}
    & \bf Train & \bf Val. & \bf Score\\
    \midrule
    Training data      & 0.0050 & 0.0120 & 3.22 \\
    MLE$^\dagger$      & 0.0100 & 0.0194 & \bf{3.43} \\
    \midrule
    SeqGAN$^\ddagger$  & 0.1234 & 0.1422 & 6.09 \\
    MaliGAN$^\ddagger$ & 0.1280 & 0.1504 & 6.30 \\
    RankGAN$^\ddagger$ & 0.1418 & 0.1431 & 5.76 \\
    LeakGAN$^\ddagger$ & 0.0718 & 0.0691 & 4.90 \\
    RelGAN$^\ddagger$  & 0.0462 & 0.0408 & 3.49 \\
    \midrule
    ScratchGAN         & 0.0301 & 0.0390 & 4,96 \\
    ScratchGAN         & 0.0153 & 0.0194 & 4.46 \\
    ($N=512$) \\
    \midrule
    TaylorGAN          & 0.0105 & \bf{0.0149} & 4.02 \\
    \bottomrule
\end{tabular}
